Near complete laser-induced modulation of the ferromagnetic-antiferromagnetic phase fraction in FeRh films

With its huge entropy change and a strong interplay between magnetic order, structural and electrical properties, the first-order antiferromagnetic/ferromagnetic phase transition is a paradigmatic example of the multicaloric effect. The unraveling of the physics underlying the phase transition needs a better understanding of the thermal hysteresis of FeRh within the AF-FM phase coexistence region. In this work, we compare the effect of two very different types of thermal cycling on the hysteresis of the magnetic order: quasi-static heating, and cooling of the entire 195 nm thick film, and a f =100 kHz modulated heating driven by a laser focused down to a spot of about ten microns squared at the film surface. Taking advantage of the reflectivity difference between both phases to probe optically their respective fraction, we show that whereas only temperature-driven reflectivity variations ($dR/dT$, thermoreflectance) are detected in the pure phases, a huge modulation of the phase-dependent reflectance at the driving frequency $f$ is detected in the phase coexistence temperature range. This is quantitatively described as resulting from a substantial modulation of the FM fraction (up to 90% with increasing laser power. A simplified rate-independent hysteresis model with return-point-memory (RPM), represented in terms of bistable units that undergo a temperature excursion corresponding to a given laser power, reproduces very well the optically measured FM phase modulation characteristics for a broad range of temperature excursions. This offers an insight into the leading role of quenched disorder in defining thermal hysteresis in FeRh under high excitation frequency, when the material is periodically driven out-of-equilibrium.

==> Old_biblio.tex <==
\begin{thebibliography}{69}%
\makeatletter
\providecommand \@ifxundefined [1]{%
 \@ifx{#1\undefined}
}%
\providecommand \@ifnum [1]{%
 \ifnum #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \@ifx [1]{%
 \ifx #1\expandafter \@firstoftwo
 \else \expandafter \@secondoftwo
 \fi
}%
\providecommand \natexlab [1]{#1}%
\providecommand \enquote  [1]{``#1''}%
\providecommand \bibnamefont  [1]{#1}%
\providecommand \bibfnamefont [1]{#1}%
\providecommand \citenamefont [1]{#1}%
\providecommand \href@noop [0]{\@secondoftwo}%
\providecommand \href [0]{\begingroup \@sanitize@url \@href}%
\providecommand \@href[1]{\@@startlink{#1}\@@href}%
\providecommand \@@href[1]{\endgroup#1\@@endlink}%
\providecommand \@sanitize@url [0]{\catcode `\\12\catcode `\$12\catcode `\&12\catcode `\#12\catcode `\^12\catcode `\_12\catcode `\%12\relax}%
\providecommand \@@startlink[1]{}%
\providecommand \@@endlink[0]{}%
\providecommand \url  [0]{\begingroup\@sanitize@url \@url }%
\providecommand \@url [1]{\endgroup\@href {#1}{\urlprefix }}%
\providecommand \urlprefix  [0]{URL }%
\providecommand \Eprint [0]{\href }%
\providecommand \doibase [0]{https://doi.org/}%
\providecommand \selectlanguage [0]{\@gobble}%
\providecommand \bibinfo  [0]{\@secondoftwo}%
\providecommand \bibfield  [0]{\@secondoftwo}%
\providecommand \translation [1]{[#1]}%
\providecommand \BibitemOpen [0]{}%
\providecommand \bibitemStop [0]{}%
\providecommand \bibitemNoStop [0]{.\EOS\space}%
\providecommand \EOS [0]{\spacefactor3000\relax}%
\providecommand \BibitemShut  [1]{\csname bibitem#1\endcsname}%
\let\auto@bib@innerbib\@empty
%</preamble>
\bibitem [{\citenamefont {Fallot}(1938)}]{Fallot1938}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Fallot}},\ }\bibfield  {title} {\bibinfo {title} {Les alliages du fer avec les m{\'e}taux de la famille du platine},\ }in\ \href {https://doi.org/10.1051/anphys/193811100291} {\emph {\bibinfo {booktitle} {Ann. Phys.}}},\ Vol.~\bibinfo {volume} {11}\ (\bibinfo {year} {1938})\ pp.\ \bibinfo {pages} {291--332}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fallot}\ and\ \citenamefont {Hocart}(1939)}]{Fallot1939-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Fallot}}\ and\ \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Hocart}},\ }\bibfield  {title} {\bibinfo {title} {Sur l’apparition du ferromagn{\'e}tisme par {\'e}l{\'e}vation de temp{\'e}rature dans des alliages de fer et de rhodium},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Rev. Sci}\ }\textbf {\bibinfo {volume} {77}},\ \bibinfo {pages} {498} (\bibinfo {year} {1939})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lewis}\ \emph {et~al.}(2016)\citenamefont {Lewis}, \citenamefont {Marrows},\ and\ \citenamefont {Langridge}}]{Lewis2016-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Lewis}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Marrows}},\ and\ \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Langridge}},\ }\bibfield  {title} {\bibinfo {title} {Coupled magnetic, structural, and electronic phase transitions in {FeRh}},\ }\href {https://doi.org/10.1088/0022-3727/49/32/323002} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. D: Appl. Phys.}\ }\textbf {\bibinfo {volume} {49}},\ \bibinfo {pages} {323002} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lyubina}(2017)}]{Lyubina_2017}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Lyubina}},\ }\bibfield  {title} {\bibinfo {title} {Magnetocaloric materials for energy efficient cooling},\ }\href {https://doi.org/10.1088/1361-6463/50/5/053002} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. D: Appl. Phys.}\ }\textbf {\bibinfo {volume} {50}},\ \bibinfo {pages} {053002} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Stern-Taulats}\ \emph {et~al.}(2017)\citenamefont {Stern-Taulats}, \citenamefont {Cast{\'a}n}, \citenamefont {Planes}, \citenamefont {Lewis}, \citenamefont {Barua}, \citenamefont {Pramanick}, \citenamefont {Majumdar},\ and\ \citenamefont {Ma{\~n}osa}}]{Stern-Taulats2017-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Stern-Taulats}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Cast{\'a}n}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Planes}}, \bibinfo {author} {\bibfnamefont {L.~H.}\ \bibnamefont {Lewis}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Barua}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Pramanick}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Majumdar}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Ma{\~n}osa}},\ }\bibfield  {title} {\bibinfo {title} {Giant multicaloric response of bulk {Fe}\textsubscript{49}{Rh}\textsubscript{51}},\ }\href {https://doi.org/10.1103/PhysRevB.95.104424} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {95}},\ \bibinfo {pages} {104424} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Maat}\ \emph {et~al.}(2005)\citenamefont {Maat}, \citenamefont {Thiele},\ and\ \citenamefont {Fullerton}}]{Maat2005-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Maat}}, \bibinfo {author} {\bibfnamefont {J.-U.}\ \bibnamefont {Thiele}},\ and\ \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}},\ }\bibfield  {title} {\bibinfo {title} {Temperature and field hysteresis of the antiferromagnetic-to-ferromagnetic phase transition in epitaxial ferh films},\ }\href {https://doi.org/https://doi.org/10.1103/PhysRevB.72.214432} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {72}},\ \bibinfo {pages} {214432} (\bibinfo {year} {2005})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Uhlíř}\ \emph {et~al.}(2016)\citenamefont {Uhlíř}, \citenamefont {Arregi},\ and\ \citenamefont {Fullerton}}]{Uhlir2016}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhlíř}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}},\ and\ \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}},\ }\bibfield  {title} {\bibinfo {title} {Colossal magnetic phase transition asymmetry in mesoscale {FeRh} stripes},\ }\href {https://doi.org/10.1038/ncomms13113} {\bibfield  {journal} {\bibinfo  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {7}},\ \bibinfo {pages} {13113} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {De~Vries}\ \emph {et~al.}(2014)\citenamefont {De~Vries}, \citenamefont {Loving}, \citenamefont {McLaren}, \citenamefont {Brydson}, \citenamefont {Liu}, \citenamefont {Langridge}, \citenamefont {Lewis},\ and\ \citenamefont {Marrows}}]{deVries2014-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {De~Vries}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Loving}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {McLaren}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Brydson}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Liu}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Langridge}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Lewis}},\ and\ \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Marrows}},\ }\bibfield  {title} {\bibinfo {title} {Asymmetric “melting” and “freezing” kinetics of the magnetostructural phase transition in {B2}-ordered {FeRh} epilayers},\ }\href {https://doi.org/https://doi.org/10.1063/1.4883369} {\bibfield  {journal} {\bibinfo  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {104}},\ \bibinfo {pages} {232407} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Arregi}\ \emph {et~al.}(2020)\citenamefont {Arregi}, \citenamefont {Caha},\ and\ \citenamefont {Uhlíř}}]{Arregi2020a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Caha}},\ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhlíř}},\ }\bibfield  {title} {\bibinfo {title} {Evolution of strain across the magnetostructural phase transition in epitaxial {FeRh} films on different substrates},\ }\href {https://doi.org/10.1103/PhysRevB.101.174413} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {101}},\ \bibinfo {pages} {174413} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cherifi}\ \emph {et~al.}(2014)\citenamefont {Cherifi}, \citenamefont {Ivanovskaya}, \citenamefont {Phillips}, \citenamefont {Zobelli}, \citenamefont {Infante}, \citenamefont {Jacquet}, \citenamefont {Garcia}, \citenamefont {Fusil}, \citenamefont {Briddon}, \citenamefont {Guiblin} \emph {et~al.}}]{Cherifi2014-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Cherifi}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Ivanovskaya}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Phillips}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Zobelli}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Infante}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Jacquet}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Garcia}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Fusil}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Briddon}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Guiblin}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {Electric-field control of magnetic order above room temperature},\ }\href {https://doi.org/10.1038/nmat3870} {\bibfield  {journal} {\bibinfo  {journal} {Nat. Mater.}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages} {345} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Loving}\ \emph {et~al.}(2017)\citenamefont {Loving}, \citenamefont {Barua}, \citenamefont {Le~Gra{\"e}t}, \citenamefont {Kinane}, \citenamefont {Heiman}, \citenamefont {Langridge}, \citenamefont {Marrows},\ and\ \citenamefont {Lewis}}]{Loving2017-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Loving}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Barua}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Le~Gra{\"e}t}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Kinane}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Heiman}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Langridge}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Marrows}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Lewis}},\ }\bibfield  {title} {\bibinfo {title} {Strain-tuning of the magnetocaloric transition temperature in model {FeRh} films},\ }\href {https://doi.org/10.1088/1361-6463/aa9d1f} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. D: Appl. Phys.}\ }\textbf {\bibinfo {volume} {51}},\ \bibinfo {pages} {024003} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Thiele}\ \emph {et~al.}(2003)\citenamefont {Thiele}, \citenamefont {Maat},\ and\ \citenamefont {Fullerton}}]{Thiele2003-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.-U.}\ \bibnamefont {Thiele}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Maat}},\ and\ \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}},\ }\bibfield  {title} {\bibinfo {title} {{FeRh}/{FePt} exchange spring films for thermally assisted magnetic recording media},\ }\href {https://doi.org/10.1063/1.1571232} {\bibfield  {journal} {\bibinfo  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {82}},\ \bibinfo {pages} {2859} (\bibinfo {year} {2003})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Marti}\ \emph {et~al.}(2014)\citenamefont {Marti}, \citenamefont {Fina}, \citenamefont {Frontera}, \citenamefont {Liu}, \citenamefont {Wadley}, \citenamefont {He}, \citenamefont {Paull}, \citenamefont {Clarkson}, \citenamefont {Kudrnovsk{\`y}}, \citenamefont {Turek} \emph {et~al.}}]{Marti2014-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Marti}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Fina}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Frontera}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Liu}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Wadley}}, \bibinfo {author} {\bibfnamefont {Q.}~\bibnamefont {He}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Paull}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Clarkson}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Kudrnovsk{\`y}}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Turek}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {Room-temperature antiferromagnetic memory resistor},\ }\href {https://doi.org/10.1038/NMAT3861} {\bibfield  {journal} {\bibinfo  {journal} {Nat. Mater.}\ }\textbf {\bibinfo {volume} {13}},\ \bibinfo {pages} {367} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mei}\ \emph {et~al.}(2020)\citenamefont {Mei}, \citenamefont {Gray}, \citenamefont {Tang}, \citenamefont {Schubert}, \citenamefont {Werder}, \citenamefont {Bartell}, \citenamefont {Ralph}, \citenamefont {Fuchs},\ and\ \citenamefont {Schlom}}]{Mei2020a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~B.}\ \bibnamefont {Mei}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Gray}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Tang}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Schubert}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Werder}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Bartell}}, \bibinfo {author} {\bibfnamefont {D.~C.}\ \bibnamefont {Ralph}}, \bibinfo {author} {\bibfnamefont {G.~D.}\ \bibnamefont {Fuchs}},\ and\ \bibinfo {author} {\bibfnamefont {D.~G.}\ \bibnamefont {Schlom}},\ }\bibfield  {title} {\bibinfo {title} {{Local Photothermal Control of Phase Transitions for On‐Demand Room‐Temperature Rewritable Magnetic Patterning}},\ }\href {https://doi.org/10.1002/adma.202001080} {\bibfield  {journal} {\bibinfo  {journal} {Adv. Mater.}\ }\textbf {\bibinfo {volume} {32}},\ \bibinfo {pages} {2001080} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Kouvel}\ and\ \citenamefont {Hartelius}(1962)}]{Kouvel1962-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Kouvel}}\ and\ \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Hartelius}},\ }\bibfield  {title} {\bibinfo {title} {Anomalous magnetic moments and transformations in the ordered alloy {FeRh}},\ }in\ \href@noop {} {\emph {\bibinfo {booktitle} {Proceedings of the Seventh Conference on Magnetism and Magnetic Materials}}}\ (\bibinfo {organization} {Springer},\ \bibinfo {year} {1962})\ pp.\ \bibinfo {pages} {1343--1344}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wu}\ \emph {et~al.}(2024)\citenamefont {Wu}, \citenamefont {Liu}, \citenamefont {Gao}, \citenamefont {Mi}, \citenamefont {Jia}, \citenamefont {Wang}, \citenamefont {Liu}, \citenamefont {Zhang}, \citenamefont {Wei}, \citenamefont {Wang} \emph {et~al.}}]{Wu2024-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Wu}}, \bibinfo {author} {\bibfnamefont {Q.}~\bibnamefont {Liu}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Gao}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Mi}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Jia}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Wang}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Liu}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Zhang}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Wei}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Wang}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {Acoustic {W}ave-{I}nduced {FeRh} {M}agnetic {P}hase {T}ransition and {I}ts {A}pplication in {A}ntiferromagnetic {P}attern {W}riting and {E}rasing},\ }\href {https://doi.org/10.1021/acsnano.3c11619} {\bibfield  {journal} {\bibinfo  {journal} {ACS Nano}\ }\textbf {\bibinfo {volume} {18}},\ \bibinfo {pages} {12134} (\bibinfo {year} {2024})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Saidl}\ \emph {et~al.}(2016)\citenamefont {Saidl}, \citenamefont {Brajer}, \citenamefont {Hor{\'{a}}k}, \citenamefont {Reichlov{\'{a}}}, \citenamefont {V{\'{y}}born{\'{y}}}, \citenamefont {Veis}, \citenamefont {Janda}, \citenamefont {Troj{\'{a}}nek}, \citenamefont {Mary{\v{s}}ko}, \citenamefont {Fina}, \citenamefont {Marti}, \citenamefont {Jungwirth},\ and\ \citenamefont {N{\v{e}}mec}}]{Saidl2016a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Saidl}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Brajer}}, \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Hor{\'{a}}k}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Reichlov{\'{a}}}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {V{\'{y}}born{\'{y}}}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Veis}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Janda}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Troj{\'{a}}nek}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Mary{\v{s}}ko}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Fina}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Marti}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Jungwirth}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {N{\v{e}}mec}},\ }\bibfield  {title} {\bibinfo {title} {{Investigation of magneto-structural phase transition in FeRh by reflectivity and transmittance
  measurements in visible and near-infrared spectral region}},\ }\href {https://doi.org/10.1088/1367-2630/18/8/083017} {\bibfield  {journal} {\bibinfo  {journal} {New J. Phys.}\ }\textbf {\bibinfo {volume} {18}},\ \bibinfo {pages} {083017} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Staunton}\ \emph {et~al.}(2014)\citenamefont {Staunton}, \citenamefont {Banerjee}, \citenamefont {Dias}, \citenamefont {Deak},\ and\ \citenamefont {Szunyogh}}]{Staunton2014-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~B.}\ \bibnamefont {Staunton}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Banerjee}}, \bibinfo {author} {\bibfnamefont {M.~d.~S.}\ \bibnamefont {Dias}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Deak}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Szunyogh}},\ }\bibfield  {title} {\bibinfo {title} {Fluctuating local moments, itinerant electrons, and the magnetocaloric effect: Compositional hypersensitivity of {FeRh}},\ }\href {https://doi.org/10.1103/PhysRevB.89.054427} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {89}},\ \bibinfo {pages} {054427} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Aubert}\ \emph {et~al.}(2024)\citenamefont {Aubert}, \citenamefont {Skokov}, \citenamefont {Rogalev}, \citenamefont {Chirkova}, \citenamefont {Beckmann}, \citenamefont {Maccari}, \citenamefont {Dilmieva}, \citenamefont {Wilhelm}, \citenamefont {Nassif}, \citenamefont {Diop}, \citenamefont {Bruder}, \citenamefont {L{\"o}fstrand}, \citenamefont {Primetzhofer}, \citenamefont {Sahlberg}, \citenamefont {Adabifiroozjaei}, \citenamefont {Molina-Luna}, \citenamefont {Gomez}, \citenamefont {Eggert}, \citenamefont {Ollefs}, \citenamefont {Wende},\ and\ \citenamefont {Gutfleisch}}]{Aubert-2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Aubert}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Skokov}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Rogalev}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Chirkova}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Beckmann}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Maccari}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Dilmieva}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Wilhelm}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Nassif}}, \bibinfo {author} {\bibfnamefont {L.~V.~B.}\ \bibnamefont {Diop}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Bruder}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {L{\"o}fstrand}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Primetzhofer}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Sahlberg}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Adabifiroozjaei}}, \bibinfo {author} {\bibfnamefont
  {L.}~\bibnamefont {Molina-Luna}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Gomez}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Eggert}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Ollefs}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Wende}},\ and\ \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Gutfleisch}},\ }\bibfield  {title} {\bibinfo {title} {Residual ferromagnetic regions affecting the first-order phase transition in off-stoichiometric fe–rh},\ }\href {https://doi.org/10.1021/acsami.4c12432} {\bibfield  {journal} {\bibinfo  {journal} {ACS Applied Materials \& Interfaces}\ }\textbf {\bibinfo {volume} {16}},\ \bibinfo {pages} {62358} (\bibinfo {year} {2024})},\ \bibinfo {note} {pMID: 39472303},\ \Eprint {https://arxiv.org/abs/https://doi.org/10.1021/acsami.4c12432} {https://doi.org/10.1021/acsami.4c12432} \BibitemShut {NoStop}%
\bibitem [{\citenamefont {Arregi}\ \emph {et~al.}(2023)\citenamefont {Arregi}, \citenamefont {Ringe}, \citenamefont {Hajdu{\v{c}}ek}, \citenamefont {Gomonay}, \citenamefont {Moln{\'a}r}, \citenamefont {Jaskowiec},\ and\ \citenamefont {Uhl{\'\i}{\v{r}}}}]{Arregi2023-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Ringe}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Hajdu{\v{c}}ek}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Gomonay}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Moln{\'a}r}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Jaskowiec}},\ and\ \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl{\'\i}{\v{r}}}},\ }\bibfield  {title} {\bibinfo {title} {Magnetic-field-controlled growth of magnetoelastic phase domains in {FeRh}},\ }\href {https://doi.org/10.1088/2515-7639/acce6f} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. Mater.}\ }\textbf {\bibinfo {volume} {6}},\ \bibinfo {pages} {034003} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Thiele}\ \emph {et~al.}(2004)\citenamefont {Thiele}, \citenamefont {Buess},\ and\ \citenamefont {Back}}]{Thiele2004b}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~U.}\ \bibnamefont {Thiele}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Buess}},\ and\ \bibinfo {author} {\bibfnamefont {C.~H.}\ \bibnamefont {Back}},\ }\bibfield  {title} {\bibinfo {title} {{Spin dynamics of the antiferromagnetic-to-ferromagnetic phase transition in FeRh on a sub-picosecond time scale}},\ }\href {https://doi.org/10.1063/1.1799244} {\bibfield  {journal} {\bibinfo  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {85}},\ \bibinfo {pages} {2857} (\bibinfo {year} {2004})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Ju}\ \emph {et~al.}(2004)\citenamefont {Ju}, \citenamefont {Hohlfeld}, \citenamefont {Bergman}, \citenamefont {{Van Deveerdonk}}, \citenamefont {Mryasov}, \citenamefont {Kim}, \citenamefont {Wu}, \citenamefont {Weller},\ and\ \citenamefont {Koopmans}}]{Ju2004}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Ju}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Hohlfeld}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Bergman}}, \bibinfo {author} {\bibfnamefont {R.~J.~M.}\ \bibnamefont {{Van Deveerdonk}}}, \bibinfo {author} {\bibfnamefont {O.~N.}\ \bibnamefont {Mryasov}}, \bibinfo {author} {\bibfnamefont {J.~Y.}\ \bibnamefont {Kim}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Wu}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Weller}},\ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Koopmans}},\ }\bibfield  {title} {\bibinfo {title} {{Ultrafast generation of ferromagnetic order via a laser-induced phase transformation in FeRh thin films}},\ }\href {https://doi.org/10.1103/PhysRevLett.93.197403} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {93}},\ \bibinfo {pages} {197403} (\bibinfo {year} {2004})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bergman}\ \emph {et~al.}(2006)\citenamefont {Bergman}, \citenamefont {Ju}, \citenamefont {Hohlfeld}, \citenamefont {van~de Veerdonk}, \citenamefont {Kim}, \citenamefont {Wu}, \citenamefont {Weller},\ and\ \citenamefont {Koopmans}}]{Bergman2006}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Bergman}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Ju}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Hohlfeld}}, \bibinfo {author} {\bibfnamefont {R.~J.~M.}\ \bibnamefont {van~de Veerdonk}}, \bibinfo {author} {\bibfnamefont {J.-Y.}\ \bibnamefont {Kim}}, \bibinfo {author} {\bibfnamefont {X.}~\bibnamefont {Wu}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Weller}},\ and\ \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Koopmans}},\ }\bibfield  {title} {\bibinfo {title} {{Identifying growth mechanisms for laser-induced magnetization in FeRh}},\ }\href {https://doi.org/10.1103/PhysRevB.73.060407} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {73}},\ \bibinfo {pages} {060407} (\bibinfo {year} {2006})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Radu}\ \emph {et~al.}(2010)\citenamefont {Radu}, \citenamefont {Stamm}, \citenamefont {Pontius}, \citenamefont {Kachel}, \citenamefont {Ramm}, \citenamefont {Thiele}, \citenamefont {D{\"{u}}rr},\ and\ \citenamefont {Back}}]{Radu2010}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Radu}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Stamm}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont {Pontius}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Kachel}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Ramm}}, \bibinfo {author} {\bibfnamefont {J.-U.}\ \bibnamefont {Thiele}}, \bibinfo {author} {\bibfnamefont {H.~A.}\ \bibnamefont {D{\"{u}}rr}},\ and\ \bibinfo {author} {\bibfnamefont {C.~H.}\ \bibnamefont {Back}},\ }\bibfield  {title} {\bibinfo {title} {{Laser-induced generation and quenching of magnetization on FeRh studied with time-resolved x-ray magnetic circular dichroism}},\ }\href {https://doi.org/10.1103/PhysRevB.81.104415} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {81}},\ \bibinfo {pages} {104415} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Quirin}\ \emph {et~al.}(2012)\citenamefont {Quirin}, \citenamefont {Vattilana}, \citenamefont {Shymanovich}, \citenamefont {El-Kamhawy}, \citenamefont {Tarasevitch}, \citenamefont {Hohlfeld}, \citenamefont {von~der Linde},\ and\ \citenamefont {Sokolowski-Tinten}}]{Quirin2012a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Quirin}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Vattilana}}, \bibinfo {author} {\bibfnamefont {U.}~\bibnamefont {Shymanovich}}, \bibinfo {author} {\bibfnamefont {A.-E.}\ \bibnamefont {El-Kamhawy}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Tarasevitch}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Hohlfeld}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {von~der Linde}},\ and\ \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Sokolowski-Tinten}},\ }\bibfield  {title} {\bibinfo {title} {{Structural dynamics in FeRh during a laser-induced metamagnetic phase transition}},\ }\href {https://doi.org/10.1103/PhysRevB.85.020103} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {85}},\ \bibinfo {pages} {020103} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mariager}\ \emph {et~al.}(2012)\citenamefont {Mariager}, \citenamefont {Pressacco}, \citenamefont {Ingold}, \citenamefont {Caviezel}, \citenamefont {M{\"o}hr-Vorobeva}, \citenamefont {Beaud}, \citenamefont {Johnson}, \citenamefont {Milne}, \citenamefont {Mancini}, \citenamefont {Moyerman} \emph {et~al.}}]{Mariager2012-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {S.~O.}\ \bibnamefont {Mariager}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Pressacco}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Ingold}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Caviezel}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {M{\"o}hr-Vorobeva}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Beaud}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Johnson}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Milne}}, \bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Mancini}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Moyerman}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {Structural and magnetic dynamics of a laser induced phase transition in {FeRh}},\ }\href {https://doi.org/10.1103/PhysRevLett.108.087201} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {108}},\ \bibinfo {pages} {087201} (\bibinfo {year} {2012})}\BibitemShut
  {NoStop}%
\bibitem [{\citenamefont {Pressacco}\ \emph {et~al.}(2018)\citenamefont {Pressacco}, \citenamefont {Uhl{\'{i}}ř}, \citenamefont {Gatti}, \citenamefont {Nicolaou}, \citenamefont {Bendounan}, \citenamefont {Arregi}, \citenamefont {Patel}, \citenamefont {Fullerton}, \citenamefont {Krizmancic},\ and\ \citenamefont {Sirotti}}]{Pressacco2018}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Pressacco}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl{\'{i}}ř}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Gatti}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Nicolaou}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Bendounan}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {S.~K.~K.}\ \bibnamefont {Patel}}, \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Krizmancic}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Sirotti}},\ }\bibfield  {title} {\bibinfo {title} {{Laser induced phase transition in epitaxial FeRh layers studied by pump-probe valence band photoemission}},\ }\href {https://doi.org/10.1063/1.5027809} {\bibfield  {journal} {\bibinfo  {journal} {Struct. Dyn.}\ }\textbf {\bibinfo {volume} {5}},\ \bibinfo {pages} {034501} (\bibinfo {year}
  {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pressacco}\ \emph {et~al.}(2021)\citenamefont {Pressacco}, \citenamefont {Sangalli}, \citenamefont {Uhl{\'{i}}{\v{r}}}, \citenamefont {Kutnyakhov}, \citenamefont {Arregi}, \citenamefont {Agustsson}, \citenamefont {Brenner}, \citenamefont {Redlin}, \citenamefont {Heber}, \citenamefont {Vasilyev}, \citenamefont {Demsar}, \citenamefont {Sch{\"{o}}nhense}, \citenamefont {Gatti}, \citenamefont {Marini}, \citenamefont {Wurth},\ and\ \citenamefont {Sirotti}}]{Pressacco2021}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Pressacco}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Sangalli}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl{\'{i}}{\v{r}}}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Kutnyakhov}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {S.~Y.}\ \bibnamefont {Agustsson}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Brenner}}, \bibinfo {author} {\bibfnamefont {H.}~\bibnamefont {Redlin}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Heber}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Vasilyev}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Demsar}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Sch{\"{o}}nhense}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Gatti}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Marini}}, \bibinfo {author} {\bibfnamefont {W.}~\bibnamefont {Wurth}},\ and\ \bibinfo {author}
  {\bibfnamefont {F.}~\bibnamefont {Sirotti}},\ }\bibfield  {title} {\bibinfo {title} {{Subpicosecond metamagnetic phase transition in FeRh driven by non-equilibrium electron dynamics}},\ }\href {https://doi.org/10.1038/s41467-021-25347-3} {\bibfield  {journal} {\bibinfo  {journal} {Nat. Commun.}\ }\textbf {\bibinfo {volume} {12}},\ \bibinfo {pages} {5088} (\bibinfo {year} {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mattern}\ \emph {et~al.}(2024)\citenamefont {Mattern}, \citenamefont {Jarecki}, \citenamefont {Arregi}, \citenamefont {Uhl{\'{i}}{\v{r}}}, \citenamefont {R{\"{o}}ssle},\ and\ \citenamefont {Bargheer}}]{Mattern2024a}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Mattern}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Jarecki}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl{\'{i}}{\v{r}}}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {R{\"{o}}ssle}},\ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Bargheer}},\ }\bibfield  {title} {\bibinfo {title} {{Speed limits of the laser-induced phase transition in FeRh}},\ }\href {https://doi.org/10.1063/5.0206095} {\bibfield  {journal} {\bibinfo  {journal} {APL Mater.}\ }\textbf {\bibinfo {volume} {12}},\ \bibinfo {pages} {051124} (\bibinfo {year} {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Dolgikh}\ \emph {et~al.}(2025)\citenamefont {Dolgikh}, \citenamefont {Blank}, \citenamefont {Buzdakov}, \citenamefont {Li}, \citenamefont {Prabhakara}, \citenamefont {Patel}, \citenamefont {Medapalli}, \citenamefont {Fullerton}, \citenamefont {Koplak}, \citenamefont {Mentink} \emph {et~al.}}]{Dolgikh2025}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.~A.}\ \bibnamefont {Dolgikh}}, \bibinfo {author} {\bibfnamefont {T.~G.~H.}\ \bibnamefont {Blank}}, \bibinfo {author} {\bibfnamefont {A.~G.}\ \bibnamefont {Buzdakov}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Li}}, \bibinfo {author} {\bibfnamefont {K.~H.}\ \bibnamefont {Prabhakara}}, \bibinfo {author} {\bibfnamefont {S.~K.~K.}\ \bibnamefont {Patel}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Medapalli}}, \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}}, \bibinfo {author} {\bibfnamefont {O.~V.}\ \bibnamefont {Koplak}}, \bibinfo {author} {\bibfnamefont {J.~H.}\ \bibnamefont {Mentink}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {{Ultrafast emergence of ferromagnetism in antiferromagnetic FeRh in high magnetic fields}},\ }\href {https://doi.org/10.1038/s44306-024-00069-6} {\bibfield  {journal} {\bibinfo  {journal} {npj Spintronics}\ }\textbf {\bibinfo {volume} {3}},\ \bibinfo {pages} {5} (\bibinfo {year}
  {2025})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Harton}\ \emph {et~al.}(2024)\citenamefont {Harton}, \citenamefont {Ceballos-Sanchez}, \citenamefont {Unikandanunni}, \citenamefont {Gray}, \citenamefont {Bonetti}, \citenamefont {Kr{\"u}ger},\ and\ \citenamefont {Hellman}}]{Harton2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.~M.}\ \bibnamefont {Harton}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Ceballos-Sanchez}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Unikandanunni}}, \bibinfo {author} {\bibfnamefont {A.~X.}\ \bibnamefont {Gray}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Bonetti}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Kr{\"u}ger}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Hellman}},\ }\bibfield  {title} {\bibinfo {title} {Characterizing the nonequilibrium response of {FeRh} thin films using time-domain thermoreflectance},\ }\href {https://doi.org/10.1103/PhysRevB.110.094417} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {110}},\ \bibinfo {pages} {094417} (\bibinfo {year} {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Castellano}\ \emph {et~al.}(2024)\citenamefont {Castellano}, \citenamefont {Alhada-Lahbabi}, \citenamefont {Arregi}, \citenamefont {Uhl\'{\i}\ifmmode~\check{r}\else \v{r}\fi{}}, \citenamefont {Perrin}, \citenamefont {Gourdon}, \citenamefont {Fournier}, \citenamefont {Verstraete},\ and\ \citenamefont {Thevenard}}]{Castellano2024}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Castellano}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Alhada-Lahbabi}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Arregi}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl\'{\i}\ifmmode~\check{r}\else \v{r}\fi{}}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont {Perrin}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Gourdon}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Fournier}}, \bibinfo {author} {\bibfnamefont {M.~J.}\ \bibnamefont {Verstraete}},\ and\ \bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {Thevenard}},\ }\bibfield  {title} {\bibinfo {title} {Magnetic phase dependency of the thermal conductivity of {FeRh} from thermoreflectance experiments and numerical simulations},\ }\href {https://doi.org/10.1103/PhysRevMaterials.8.084411} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Mater.}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo {pages} {084411} (\bibinfo {year}
  {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Fournier}\ \emph {et~al.}(2020)\citenamefont {Fournier}, \citenamefont {Marangolo},\ and\ \citenamefont {Fretigny}}]{Fournier2020}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Fournier}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Marangolo}},\ and\ \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Fretigny}},\ }\bibfield  {title} {\bibinfo {title} {{Measurement of thermal properties of bulk materials and thin films by modulated thermoreflectance (MTR)}},\ }\href {https://doi.org/10.1063/5.0019025} {\bibfield  {journal} {\bibinfo  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {128}},\ \bibinfo {pages} {241101} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%
\bibitem [{Note1()}]{Note1}%
  \BibitemOpen
  \bibinfo {note} {Both pump and probe beams are circularly polarized when impinging the sample, and linearized back when returning towards the photodiode. A narrow interference filter in front of the detector suppresses the green pump beam.}\BibitemShut {Stop}%
\bibitem [{Note2()}]{Note2}%
  \BibitemOpen
  \bibinfo {note} {A filter cutting the green laser is placed in front of the photodiode. Prior to the experiment, the phase of the lock-in detection is adjusted by removing the filter and detecting directly the reflected pump laser flux with the photodiode.}\BibitemShut {Stop}%
\bibitem [{\citenamefont {Keavney}\ \emph {et~al.}(2018)\citenamefont {Keavney}, \citenamefont {Choi}, \citenamefont {Holt}, \citenamefont {Uhl{\'\i}{\v{r}}}, \citenamefont {Arena}, \citenamefont {Fullerton}, \citenamefont {Ryan},\ and\ \citenamefont {Kim}}]{Keavney2018-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~J.}\ \bibnamefont {Keavney}}, \bibinfo {author} {\bibfnamefont {Y.}~\bibnamefont {Choi}}, \bibinfo {author} {\bibfnamefont {M.~V.}\ \bibnamefont {Holt}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Uhl{\'\i}{\v{r}}}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Arena}}, \bibinfo {author} {\bibfnamefont {E.~E.}\ \bibnamefont {Fullerton}}, \bibinfo {author} {\bibfnamefont {P.~J.}\ \bibnamefont {Ryan}},\ and\ \bibinfo {author} {\bibfnamefont {J.-W.}\ \bibnamefont {Kim}},\ }\bibfield  {title} {\bibinfo {title} {Phase coexistence and kinetic arrest in the magnetostructural transition of the ordered alloy {F}e{R}h},\ }\href {https://doi.org/10.1038/s41598-018-20101-0} {\bibfield  {journal} {\bibinfo  {journal} {Sci. Rep.}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo {pages} {1778} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Madelung}(1905)}]{Madelung1905-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Madelung}},\ }\bibfield  {title} {\bibinfo {title} {{\"U}ber {M}agnetisierung durch schnellverlaufende {S}tr\"omeund die {W}irkungsweise des {R}utherford-{M}arconischen {M}agnetdetektors},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Ann. Phys.}\ }\textbf {\bibinfo {volume} {17}},\ \bibinfo {pages} {861 } (\bibinfo {year} {1905})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Brokate}\ and\ \citenamefont {Sprekels}(2012)}]{Brokate2012-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Brokate}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Sprekels}},\ }\href@noop {} {\emph {\bibinfo {title} {Hysteresis and phase transitions}}},\ \bibinfo {series} {Applied MAthematical Sciences (AMS)}, Vol.\ \bibinfo {volume} {121}\ (\bibinfo  {publisher} {Springer Science},\ \bibinfo {address} {New York, NY},\ \bibinfo {year} {2012})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pierce}\ \emph {et~al.}(2007)\citenamefont {Pierce}, \citenamefont {Buechler}, \citenamefont {Sorensen}, \citenamefont {Kevan}, \citenamefont {Jagla}, \citenamefont {Deutsch}, \citenamefont {Mai}, \citenamefont {Narayan}, \citenamefont {Davies}, \citenamefont {Liu} \emph {et~al.}}]{Pierce2007-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.~S.}\ \bibnamefont {Pierce}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Buechler}}, \bibinfo {author} {\bibfnamefont {L.~B.}\ \bibnamefont {Sorensen}}, \bibinfo {author} {\bibfnamefont {S.~D.}\ \bibnamefont {Kevan}}, \bibinfo {author} {\bibfnamefont {E.~A.}\ \bibnamefont {Jagla}}, \bibinfo {author} {\bibfnamefont {J.~M.}\ \bibnamefont {Deutsch}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Mai}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Narayan}}, \bibinfo {author} {\bibfnamefont {J.~E.}\ \bibnamefont {Davies}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Liu}}, \emph {et~al.},\ }\bibfield  {title} {\bibinfo {title} {Disorder-induced magnetic memory: Experiments and theories},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {75}},\ \bibinfo {pages} {144406} (\bibinfo {year} {2007})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bertotti}(1998)}]{Bertotti1998}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Bertotti}},\ }\href@noop {} {\emph {\bibinfo {title} {{H}ysteresis in {M}agnetism: for {P}hysicists, {M}aterials {S}cientists, and {E}ngineers}}}\ (\bibinfo  {publisher} {Academic Press},\ \bibinfo {address} {San Diego},\ \bibinfo {year} {1998})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Keim}\ \emph {et~al.}(2019)\citenamefont {Keim}, \citenamefont {Paulsen}, \citenamefont {Zeravcic}, \citenamefont {Sastry},\ and\ \citenamefont {Nagel}}]{Keim2019-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.~C.}\ \bibnamefont {Keim}}, \bibinfo {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Paulsen}}, \bibinfo {author} {\bibfnamefont {Z.}~\bibnamefont {Zeravcic}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Sastry}},\ and\ \bibinfo {author} {\bibfnamefont {S.~R.}\ \bibnamefont {Nagel}},\ }\bibfield  {title} {\bibinfo {title} {Memory formation in matter},\ }\href {https://doi.org/10.1103/RevModPhys.91.035002} {\bibfield  {journal} {\bibinfo  {journal} {Rev. Mod. Phys.}\ }\textbf {\bibinfo {volume} {91}},\ \bibinfo {pages} {035002} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Baldasseroni}\ \emph {et~al.}(2012)\citenamefont {Baldasseroni}, \citenamefont {Bordel}, \citenamefont {Gray}, \citenamefont {Kaiser}, \citenamefont {Kronast}, \citenamefont {Herrero-Albillos}, \citenamefont {Schneider}, \citenamefont {Fadley},\ and\ \citenamefont {Hellman}}]{Baldasseroni2012-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Baldasseroni}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Bordel}}, \bibinfo {author} {\bibfnamefont {A.~X.}\ \bibnamefont {Gray}}, \bibinfo {author} {\bibfnamefont {A.~M.}\ \bibnamefont {Kaiser}}, \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Kronast}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Herrero-Albillos}}, \bibinfo {author} {\bibfnamefont {C.~M.}\ \bibnamefont {Schneider}}, \bibinfo {author} {\bibfnamefont {C.~S.}\ \bibnamefont {Fadley}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Hellman}},\ }\bibfield  {title} {\bibinfo {title} {Temperature-driven nucleation of ferromagnetic domains in {FeRh} thin films},\ }\href {https://doi.org/10.1063/1.4730957} {\bibfield  {journal} {\bibinfo  {journal} {Appl. Phys. Lett.}\ }\textbf {\bibinfo {volume} {100}},\ \bibinfo {pages} {262401} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Sethna}\ \emph {et~al.}(1993)\citenamefont {Sethna}, \citenamefont {Dahmen}, \citenamefont {Kartha}, \citenamefont {Krumhansl}, \citenamefont {Roberts},\ and\ \citenamefont {Shore}}]{Sethna1993-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~P.}\ \bibnamefont {Sethna}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Dahmen}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Kartha}}, \bibinfo {author} {\bibfnamefont {J.~A.}\ \bibnamefont {Krumhansl}}, \bibinfo {author} {\bibfnamefont {B.~W.}\ \bibnamefont {Roberts}},\ and\ \bibinfo {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Shore}},\ }\bibfield  {title} {\bibinfo {title} {Hysteresis and hierarchies: Dynamics of disorder-driven first-order phase transformations},\ }\href {https://doi.org/10.1103/PhysRevLett.70.3347} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf {\bibinfo {volume} {70}},\ \bibinfo {pages} {3347} (\bibinfo {year} {1993})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mungan}\ and\ \citenamefont {Terzi}(2019)}]{Mungan2019-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Mungan}}\ and\ \bibinfo {author} {\bibfnamefont {M.~M.}\ \bibnamefont {Terzi}},\ }\bibfield  {title} {\bibinfo {title} {The structure of state transition graphs in systems with return point memory: I. {G}eneral theory},\ }in\ \href {https://doi.org/10.1007/s00023-019-00807-1} {\emph {\bibinfo {booktitle} {Ann. Henri Poincar{\'e}}}},\ Vol.~\bibinfo {volume} {20}\ (\bibinfo {organization} {Springer},\ \bibinfo {year} {2019})\ pp.\ \bibinfo {pages} {2819--2872}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Koyuk}\ and\ \citenamefont {Seifert}(2019)}]{Koyuk2019-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Koyuk}}\ and\ \bibinfo {author} {\bibfnamefont {U.}~\bibnamefont {Seifert}},\ }\bibfield  {title} {\bibinfo {title} {Operationally accessible bounds on fluctuations and entropy production in periodically driven systems},\ }\href {https://doi.org/10.1103/PhysRevLett.122.230601} {\bibfield  {journal} {\bibinfo  {journal} {Physical review letters}\ }\textbf {\bibinfo {volume} {122}},\ \bibinfo {pages} {230601} (\bibinfo {year} {2019})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Preisach}(1935)}]{Preisach1935-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Preisach}},\ }\bibfield  {title} {\bibinfo {title} {{\"U}ber die magnetische {Nachwirkung}},\ }\href@noop {} {\bibfield  {journal} {\bibinfo  {journal} {Z. Phys.}\ }\textbf {\bibinfo {volume} {94}},\ \bibinfo {pages} {277} (\bibinfo {year} {1935})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {N{\'e}el}(1942)}]{Neel1942-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {N{\'e}el}},\ }\bibfield  {title} {\bibinfo {title} {Th{\'e}orie des lois d’aimantation de {L}ord {R}ayleigh et les d{\'e}placements d’une paroi isol{\'e}e},\ }\href {https://doi.org/https://hal.science/hal-02914119v1} {\bibfield  {journal} {\bibinfo  {journal} {Cahiers de physique}\ }\textbf {\bibinfo {volume} {12}},\ \bibinfo {pages} {1} (\bibinfo {year} {1942})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Biorci}\ and\ \citenamefont {Pescetti}(1958)}]{Biorci1958-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Biorci}}\ and\ \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Pescetti}},\ }\bibfield  {title} {\bibinfo {title} {Analytical theory of the behaviour of ferromagnetic materials},\ }\href {https://doi.org/10.1007/BF02745588} {\bibfield  {journal} {\bibinfo  {journal} {Nuovo Cimento}\ }\textbf {\bibinfo {volume} {7}},\ \bibinfo {pages} {829} (\bibinfo {year} {1958})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Wohlfarth}(1964)}]{Wohlfarth1964-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Wohlfarth}},\ }\bibfield  {title} {\bibinfo {title} {A review of the problem of fine-particle interactions with special reference to magnetic recording},\ }\href {https://doi.org/10.1063/1.1713475} {\bibfield  {journal} {\bibinfo  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {35}},\ \bibinfo {pages} {783} (\bibinfo {year} {1964})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Porteseil}\ \emph {et~al.}(1977)\citenamefont {Porteseil}, \citenamefont {Vergne},\ and\ \citenamefont {Cotillard}}]{Porteseil1977-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Porteseil}}, \bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Vergne}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Cotillard}},\ }\bibfield  {title} {\bibinfo {title} {D{\'e}placements d'une paroi de {B}loch {\`a} 180° dans un monocristal de fer-silicium},\ }\href {https://doi.org/10.1051/jphys:0197700380120154100} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys.}\ }\textbf {\bibinfo {volume} {38}},\ \bibinfo {pages} {1541} (\bibinfo {year} {1977})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mayergoyz}(1986)}]{Mayergoyz1986-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Mayergoyz}},\ }\bibfield  {title} {\bibinfo {title} {Mathematical models of hysteresis},\ }\href {https://doi.org/10.1109/TMAG.1986.1064347} {\bibfield  {journal} {\bibinfo  {journal} {IEEE Trans. Magn.}\ }\textbf {\bibinfo {volume} {22}},\ \bibinfo {pages} {603} (\bibinfo {year} {1986})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Basso}\ \emph {et~al.}(2007)\citenamefont {Basso}, \citenamefont {Sasso},\ and\ \citenamefont {LoBue}}]{Basso2007}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Basso}}, \bibinfo {author} {\bibfnamefont {C.~P.}\ \bibnamefont {Sasso}},\ and\ \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {LoBue}},\ }\bibfield  {title} {\bibinfo {title} {Thermodynamic aspects of first-order phase transformations with hysteresis in magnetic materials},\ }\href {https://doi.org/https://doi.org/10.1016/j.jmmm.2007.03.177} {\bibfield  {journal} {\bibinfo  {journal} {J. Magn. Magn. Mater.}\ }\textbf {\bibinfo {volume} {316}},\ \bibinfo {pages} {262} (\bibinfo {year} {2007})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Bertotti}\ \emph {et~al.}(2006)\citenamefont {Bertotti}, \citenamefont {Basso}, \citenamefont {LoBue},\ and\ \citenamefont {Magni}}]{Bertotti2006}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Bertotti}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Basso}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {LoBue}},\ and\ \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Magni}},\ }\bibinfo {title} {{T}hermodynamics, {H}ysteresis, {M}icromagnetics}\ (\bibinfo  {publisher} {Elsevier - Academic Press},\ \bibinfo {year} {2006})\ Chap.~\bibinfo {chapter} {1}, pp.\ \bibinfo {pages} {1--106}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Planes}\ and\ \citenamefont {Ort{\'\i}n}(1992)}]{Planes1992}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Planes}}\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Ort{\'\i}n}},\ }\bibfield  {title} {\bibinfo {title} {Study of thermoelastic growth during martensitic transformations},\ }\href {https://doi.org/10.1063/1.351320} {\bibfield  {journal} {\bibinfo  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {71}},\ \bibinfo {pages} {950} (\bibinfo {year} {1992})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Mayergoyz}(2003)}]{Mayergoyz2003}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {I.~D.}\ \bibnamefont {Mayergoyz}},\ }\href@noop {} {\emph {\bibinfo {title} {Mathematical models of hysteresis and their applications}}}\ (\bibinfo  {publisher} {Elsevier Science},\ \bibinfo {address} {New York},\ \bibinfo {year} {2003})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Cornejo}\ \emph {et~al.}(1997)\citenamefont {Cornejo}, \citenamefont {LoBue}, \citenamefont {Basso}, \citenamefont {Bertotti},\ and\ \citenamefont {Missell}}]{Cornejo1997}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~R.}\ \bibnamefont {Cornejo}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {LoBue}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Basso}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Bertotti}},\ and\ \bibinfo {author} {\bibfnamefont {F.~P.}\ \bibnamefont {Missell}},\ }\bibfield  {title} {\bibinfo {title} {Moving preisach model analysis of nanocrystalline {S}m{F}e{C}o},\ }\href {https://doi.org/10.1063/1.364608} {\bibfield  {journal} {\bibinfo  {journal} {J. Appl. Phys.}\ }\textbf {\bibinfo {volume} {81}},\ \bibinfo {pages} {5588} (\bibinfo {year} {1997})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Lo~Bue}\ \emph {et~al.}(1998)\citenamefont {Lo~Bue}, \citenamefont {Basso}, \citenamefont {Beatrice},\ and\ \citenamefont {Tiberto}}]{LoBue1998}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Lo~Bue}}, \bibinfo {author} {\bibfnamefont {V.}~\bibnamefont {Basso}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Beatrice}},\ and\ \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Tiberto}},\ }\bibfield  {title} {\bibinfo {title} {Description of magnetic hardening in nanocrystalline {F}e{Z}r{B}{C}u alloy using the preisach model of hysteresis},\ }\href {https://doi.org/10.1051/jp4:1998275} {\bibfield  {journal} {\bibinfo  {journal} {J. Phys. Iv}\ }\textbf {\bibinfo {volume} {8}},\ \bibinfo {pages} {323} (\bibinfo {year} {1998})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Pike}(2003)}]{Pike2003-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.~R.}\ \bibnamefont {Pike}},\ }\bibfield  {title} {\bibinfo {title} {First-order reversal-curve diagrams and reversible magnetization},\ }\href {https://doi.org/10.1103/PhysRevB.68.104424} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {68}},\ \bibinfo {pages} {104424} (\bibinfo {year} {2003})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Zhou}\ \emph {et~al.}(2010)\citenamefont {Zhou}, \citenamefont {Basu}, \citenamefont {Friedman}, \citenamefont {Finkel}, \citenamefont {Yeheskel},\ and\ \citenamefont {Barsoum}}]{Zhou2010-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~G.}\ \bibnamefont {Zhou}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Basu}}, \bibinfo {author} {\bibfnamefont {G.}~\bibnamefont {Friedman}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Finkel}}, \bibinfo {author} {\bibfnamefont {O.}~\bibnamefont {Yeheskel}},\ and\ \bibinfo {author} {\bibfnamefont {M.~W.}\ \bibnamefont {Barsoum}},\ }\bibfield  {title} {\bibinfo {title} {Hysteresis in kinking nonlinear elastic solids and the {P}reisach-{M}ayergoyz model},\ }\href {https://doi.org/10.1103/PhysRevB.82.094105} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. B}\ }\textbf {\bibinfo {volume} {82}},\ \bibinfo {pages} {094105} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Komlev}\ \emph {et~al.}(2021)\citenamefont {Komlev}, \citenamefont {Karpenkov}, \citenamefont {Kiselev}, \citenamefont {Ilina}, \citenamefont {Chirkova}, \citenamefont {Gimaev}, \citenamefont {Usami}, \citenamefont {Taniyama}, \citenamefont {Zverev},\ and\ \citenamefont {Perov}}]{Komlev2021-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~S.}\ \bibnamefont {Komlev}}, \bibinfo {author} {\bibfnamefont {D.~Y.}\ \bibnamefont {Karpenkov}}, \bibinfo {author} {\bibfnamefont {D.~A.}\ \bibnamefont {Kiselev}}, \bibinfo {author} {\bibfnamefont {T.~S.}\ \bibnamefont {Ilina}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Chirkova}}, \bibinfo {author} {\bibfnamefont {R.~R.}\ \bibnamefont {Gimaev}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Usami}}, \bibinfo {author} {\bibfnamefont {T.}~\bibnamefont {Taniyama}}, \bibinfo {author} {\bibfnamefont {V.~I.}\ \bibnamefont {Zverev}},\ and\ \bibinfo {author} {\bibfnamefont {N.~S.}\ \bibnamefont {Perov}},\ }\bibfield  {title} {\bibinfo {title} {Ferromagnetic phase nucleation and its growth evolution in ferh thin films},\ }\href {https://doi.org/10.1016/j.jallcom.2021.159924} {\bibfield  {journal} {\bibinfo  {journal} {Journal of Alloys and Compounds}\ }\textbf {\bibinfo {volume} {874}},\ \bibinfo {pages} {159924} (\bibinfo {year}
  {2021})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Baldasseroni}\ \emph {et~al.}(2015)\citenamefont {Baldasseroni}, \citenamefont {Bordel}, \citenamefont {Antonakos}, \citenamefont {Scholl}, \citenamefont {Stone}, \citenamefont {Kortright},\ and\ \citenamefont {Hellman}}]{Baldasseroni2015-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Baldasseroni}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Bordel}}, \bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Antonakos}}, \bibinfo {author} {\bibfnamefont {A.}~\bibnamefont {Scholl}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Stone}}, \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Kortright}},\ and\ \bibinfo {author} {\bibfnamefont {F.}~\bibnamefont {Hellman}},\ }\bibfield  {title} {\bibinfo {title} {Temperature-driven growth of antiferromagnetic domains in thin-film ferh},\ }\href {https://doi.org/10.1088/0953-8984/27/25/256001} {\bibfield  {journal} {\bibinfo  {journal} {J. Condens. Matter Phys.}\ }\textbf {\bibinfo {volume} {27}},\ \bibinfo {pages} {256001} (\bibinfo {year} {2015})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Paulsen}\ and\ \citenamefont {Keim}(2024)}]{Paulsen2024-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~D.}\ \bibnamefont {Paulsen}}\ and\ \bibinfo {author} {\bibfnamefont {N.~C.}\ \bibnamefont {Keim}},\ }\bibfield  {title} {\bibinfo {title} {Mechanical memories in solids, from disorder to design},\ }\href {https://doi.org/10.1146/annurev-conmatphys-032822-035544} {\bibfield  {journal} {\bibinfo  {journal} {Annu. Rev. Condens. Matter Phys.}\ }\textbf {\bibinfo {volume} {16}} (\bibinfo {year} {2024})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Reichhardt}\ \emph {et~al.}(2023)\citenamefont {Reichhardt}, \citenamefont {Regev}, \citenamefont {Dahmen}, \citenamefont {Okuma},\ and\ \citenamefont {Reichhardt}}]{Reichhardt2023-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {C.}~\bibnamefont {Reichhardt}}, \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Regev}}, \bibinfo {author} {\bibfnamefont {K.}~\bibnamefont {Dahmen}}, \bibinfo {author} {\bibfnamefont {S.}~\bibnamefont {Okuma}},\ and\ \bibinfo {author} {\bibfnamefont {C.~J.~O.}\ \bibnamefont {Reichhardt}},\ }\bibfield  {title} {\bibinfo {title} {Reversible to irreversible transitions in periodic driven many-body systems and future directions for classical and quantum systems},\ }\href {https://doi.org/10.1103/PhysRevResearch.5.021001} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Res.}\ }\textbf {\bibinfo {volume} {5}},\ \bibinfo {pages} {021001} (\bibinfo {year} {2023})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {N{\'e}el}(1950)}]{Neel1950-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {L.}~\bibnamefont {N{\'e}el}},\ }\bibfield  {title} {\bibinfo {title} {Th{\'e}orie du tra{\^\i}nage magn{\'e}tique des substances massives dans le domaine de {R}ayleigh},\ }\href {https://doi.org/10.1051/jphysrad:0195000110204900} {\bibfield  {journal} {\bibinfo  {journal} {J. phys. radium}\ }\textbf {\bibinfo {volume} {11}},\ \bibinfo {pages} {49} (\bibinfo {year} {1950})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Majumdar}\ and\ \citenamefont {Regev}(2023)}]{Majumdar2023-1}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Majumdar}}\ and\ \bibinfo {author} {\bibfnamefont {I.}~\bibnamefont {Regev}},\ }\bibfield  {title} {\bibinfo {title} {Memory switching due to thermal noise in amorphous solids subject to cyclic shear},\ }\bibfield  {journal} {\bibinfo  {journal} {arXiv preprint arXiv:2310.09869}\ }\href {https://doi.org/10.48550/arXiv.2310.09869} {10.48550/arXiv.2310.09869} (\bibinfo {year} {2023})\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Richardson}\ \emph {et~al.}(1973)\citenamefont {Richardson}, \citenamefont {Melville},\ and\ \citenamefont {Ricodeau}}]{Richardson1973}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {M.}~\bibnamefont {Richardson}}, \bibinfo {author} {\bibfnamefont {D.}~\bibnamefont {Melville}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont {Ricodeau}},\ }\bibfield  {title} {\bibinfo {title} {Specific heat measurements on an fe rh alloy},\ }\href {https://doi.org/10.1016/0375-9601(73)90071-6} {\bibfield  {journal} {\bibinfo  {journal} {Physics Letters A}\ }\textbf {\bibinfo {volume} {46}},\ \bibinfo {pages} {153} (\bibinfo {year} {1973})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Hofmeister}(2014)}]{Hofmeister2014}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A.~M.}\ \bibnamefont {Hofmeister}},\ }\bibfield  {title} {\bibinfo {title} {{Thermal diffusivity and thermal conductivity of single-crystal MgO and Al2O3 and related compounds as a function of temperature}},\ }\href {https://doi.org/10.1007/s00269-014-0655-3} {\bibfield  {journal} {\bibinfo  {journal} {Phys. Chem. Miner.}\ }\textbf {\bibinfo {volume} {41}},\ \bibinfo {pages} {361} (\bibinfo {year} {2014})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Della~Torre}(1966)}]{Della-Torre1966}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {E.}~\bibnamefont {Della~Torre}},\ }\bibfield  {title} {\bibinfo {title} {Effect of interaction on the magnetization of single-domain particles},\ }\href {https://doi.org/10.1109/TAU.1966.1161852} {\bibfield  {journal} {\bibinfo  {journal} {IEEE Trans. Audio}\ }\textbf {\bibinfo {volume} {14}},\ \bibinfo {pages} {86} (\bibinfo {year} {1966})}\BibitemShut {NoStop}%
\bibitem [{\citenamefont {Killick}\ \emph {et~al.}(2012)\citenamefont {Killick}, \citenamefont {Fearnhead},\ and\ \citenamefont {Eckley}}]{Killick-2012}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont {Killick}}, \bibinfo {author} {\bibfnamefont {P.}~\bibnamefont {Fearnhead}},\ and\ \bibinfo {author} {\bibfnamefont {I.~A.}\ \bibnamefont {Eckley}},\ }\bibfield  {title} {\bibinfo {title} {Optimal detection of changepoints with a linear computational cost},\ }\href {https://doi.org/10.1080/01621459.2012.737745} {\bibfield  {journal} {\bibinfo  {journal} {Journal of the American Statistical Association}\ }\textbf {\bibinfo {volume} {107}},\ \bibinfo {pages} {1590} (\bibinfo {year} {2012})},\ \Eprint {https://arxiv.org/abs/https://doi.org/10.1080/01621459.2012.737745} {https://doi.org/10.1080/01621459.2012.737745} \BibitemShut {NoStop}%
\end{thebibliography}%
